Natlog: a Lightweight Logic Programming Language with a Neuro-symbolic Touch

We introduce Natlog, a lightweight Logic Programming language, sharing Prolog's unification-driven execution model, but with a simplified syntax and semantics. Our proof-of-concept Natlog implementation is tightly embedded in the Python-based deep-learning ecosystem with focus on content-driven indexing of ground term datasets. As an overriding of our symbolic indexing algorithm, the same function can be delegated to a neural network, serving ground facts to Natlog's resolution engine. Our open-source implementation is available as a Python package at https://pypi.org/project/natlog/ .

==> eptcsdata.tex <==
\providecommand{\firstpage}{141}
\providecommand{\publicationstatus}{A. Formisano, Y.A Liu, et al. (Eds.): International Conference on\\ Logic Programming (Technical Communications) 2021 (ICLP 2021)\\
EPTCS 345, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.345.27}{10.4204/EPTCS.345.27}}

